Effective and Efficient Dropout for Deep Convolutional Neural Networks

Convolutional Neural networks (CNNs) based applications have become ubiquitous, where proper regularization is greatly needed. To prevent large neural network models from overfitting, dropout has been widely used as an efficient regularization technique in practice. However, many recent works show that the standard dropout is ineffective or even detrimental to the training of CNNs. In this paper, we revisit this issue and examine various dropout variants in an attempt to improve existing dropout-based regularization techniques for CNNs. We attribute the failure of standard dropout to the conflict between the stochasticity of dropout and its following Batch Normalization (BN), and propose to reduce the conflict by placing dropout operations right before the convolutional operation instead of BN, or totally address this issue by replacing BN with Group Normalization (GN). We further introduce a structurally more suited dropout variant Drop-Conv2d, which provides more efficient and effective regularization for deep CNNs. These dropout variants can be readily integrated into the building blocks of CNNs and implemented in existing deep learning platforms. Extensive experiments on benchmark datasets including CIFAR, SVHN and ImageNet are conducted to compare the existing building blocks and the proposed ones with dropout training. Results show that our building blocks improve over state-of-the-art CNNs significantly, which is mainly due to the better regularization and implicit model ensemble effect.

==> bios.tex <==
\begin{IEEEbiography}[{
\includegraphics[width=1in,height=1in,clip,keepaspectratio]{bios/self.jpeg}}]
{Shaofeng Cai} received the BSc degree from the School of Electronics
Engineering and Computer Science, Peking University, China, in 2016. He is currently working towards the Ph.D. degree in School of Computing, National University of Singapore. His research interests include the areas of regularization and neural networks.
\end{IEEEbiography}
% \vspace{-5mm}
\begin{IEEEbiography}[{
\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/shuyao.jpeg}}]
{Yao Shu} received the BSc degree from Computer Science and Technology from Huazhong University of Science \& Technology, China in 2017. He is
currently a Ph.D. advised by Prof. Wang Wei at National University of Singapre (NUS).
His research interests include convex/nonconvex optimization, Bayesian Deep Learning and other Deep Learning theory such as Neural Tangent Kernel.
\end{IEEEbiography}
% \vspace{-5mm}
\begin{IEEEbiography}[{
\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/wangwei.png}}]
{Wei Wang} is an assistant professor in School of Computing, National University of Singapore (NUS). He got his BSc from Renmin University of China in 2011 and Ph.D. from NUS in 2017. His research interests include deep learning systems and applications for multimedia data. His papers were published in VLDB, ACM Multimedia, VLDBJ, TOMM. He has served as a PC member for ACM Multimedia, VLDB, ICDE and DASFAA.
\end{IEEEbiography}
% \vspace{-5mm}
\begin{IEEEbiography}[{
\includegraphics[width=1in,height=11in,clip,keepaspectratio]{bios/cg.png}}]
{Gang Chen} received the BSc, MSc and Ph.D. degrees in Computer Science and Engineering from Zhejiang University in 1993, 1995, and 1998, respectively. He is currently a professor and the dean in the College of Computer Science, Zhejiang University. His research interests include databases, information retrieval, information security, and computer-supported cooperative work. He is also the executive director of Zhejiang University Netease Joint Lab on Internet Technology. He is a member of the IEEE.
\end{IEEEbiography}
% \vspace{-5mm}
\begin{IEEEbiography}[{
\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/ooibc.png}}]
{Beng Chin Ooi} is currently a distinguished professor of Computer Science at the National University of Singapore. His research interests include database system architectures, performance issues, indexing techniques and query processing, in the context of multimedia, spatio-temporal, distributed, parallel, blockchain, and in-memory systems. He served as the editor-in-chief of the IEEE Transactions on Knowledge and Data Engineering (2009-2012), a trustee board member and the president of the VLDB Endowment (2014-2017). He is a fellow of the IEEE, ACM and Singapore National Academy of Science. He is serving as the editor-in-chief of ACM Transactions on Data Science.
\end{IEEEbiography}
% \vspace{-5mm}
\begin{IEEEbiography}[{
\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/meihui.png}}]
{Meihui Zhang} received the BEng degree in Computer Science from Harbin
Institute of Technology, China, in 2008, and Ph.D. in Computer Science from the National University of Singapore in 2013. She is currently a professor at the Beijing Institute of Technology and was an assistant professor at the Singapore University of Technology and Design (SUTD) from 2014 to 2017. Her research interests include crowd sourcing-powered data analytics, massive data integration, spatio-temporal databases, distributed systems, blockchain, and AI. She is a member of the IEEE. She has served as a vice pc-chair for VLDB'18, IEEE ICDE'18, VLDB'19, and VLDB'20. She is a winner of VLDB 2019 best paper award.
\end{IEEEbiography}

